Text is Text, No Matter What: Unifying Text Recognition using Knowledge Distillation

Text recognition remains a fundamental and extensively researched topic in computer vision, largely owing to its wide array of commercial applications. The challenging nature of the very problem however dictated a fragmentation of research efforts: Scene Text Recognition (STR) that deals with text in everyday scenes, and Handwriting Text Recognition (HTR) that tackles hand-written text. In this paper, for the first time, we argue for their unification -- we aim for a single model that can compete favourably with two separate state-of-the-art STR and HTR models. We first show that cross-utilisation of STR and HTR models trigger significant performance drops due to differences in their inherent challenges. We then tackle their union by introducing a knowledge distillation (KD) based framework. This is however non-trivial, largely due to the variable-length and sequential nature of text sequences, which renders off-the-shelf KD techniques that mostly works with global fixed-length data inadequate. For that, we propose three distillation losses all of which are specifically designed to cope with the aforementioned unique characteristics of text recognition. Empirical evidence suggests that our proposed unified model performs on par with individual models, even surpassing them in certain cases. Ablative studies demonstrate that naive baselines such as a two-stage framework, and domain adaption/generalisation alternatives do not work as well, further verifying the appropriateness of our design.

==> notes.tex <==
Most Knowledge Distillation methods give an improvement of nearly 1-2\% over their baselines. That student beats its teacher is observed only in Multilingual NMT. But in that paper the student was already behind its teacher by a small margin which was comfortable overcome by the knowledge distillation losses.

If we look at hinton's paper or "Knowledge Adaptation for Efficient Semantic Segmentation" they get an improvement of nearly 1\% only over their baselines.

Question: It is wise to show that our student performs even better than teachers? Given that the GAP between Jointly trained model and specialised models are about 15.8\% for IC15 and 5.2\% for IAM.

We have shown that using $\mathcal{L}_{logits}$ gives an improvement of 7\% but usually when $\mathcal{L}_{logits}$ are usually applied for other problems, it gives a small improvement of 1\%. This looks bad.
